Simple Disentanglement of Style and Content in Visual Representations

Learning visual representations with interpretable features, i.e., disentangled representations, remains a challenging problem. Existing methods demonstrate some success but are hard to apply to large-scale vision datasets like ImageNet. In this work, we propose a simple post-processing framework to disentangle content and style in learned representations from pre-trained vision models. We model the pre-trained features probabilistically as linearly entangled combinations of the latent content and style factors and develop a simple disentanglement algorithm based on the probabilistic model. We show that the method provably disentangles content and style features and verify its efficacy empirically. Our post-processed features yield significant domain generalization performance improvements when the distribution shift occurs due to style changes or style-related spurious correlations.

==> YK-macros.tex <==

\def\Avar{{\sf Avar}}
\def\abs#1{\left|#1\right|}
\def\innerprod#1{\left\langle#1\right\rangle}
\def\aff{{\sf aff}}
\def\argmin{{\arg\min}}
\def\argmax{{\arg\max}}
\def\avar{{\sf avar}}

\def\bA{\mathbf{A}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\bD{\mathbf{D}}
\def\bE{\mathbf{E}}
\def\bF{\mathbf{F}}
\def\bff{\mathbf{f}}
\def\bG{\mathbf{G}}
\def\bH{\mathbf{H}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bK{\mathbf{K}}
\def\bL{\mathbf{L}}
\def\bM{\mathbf{M}}
\def\bN{\mathbf{N}}
\def\bO{\mathbf{O}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bR{\mathbf{R}}
\def\bS{\mathbf{S}}
\def\bT{\mathbf{T}}
\def\bU{\mathbf{U}}
\def\bV{\mathbf{V}}
\def\bW{\mathbf{W}}
\def\bX{\mathbf{X}}
\def\bY{\mathbf{Y}}
\def\bZ{\mathbf{Z}}

\def\bGamma{{\boldsymbol\Gamma}}
\def\bDelta{{\boldsymbol\Delta}}
\def\bTheta{{\boldsymbol\Theta}}
\def\bLambda{{\boldsymbol\Lambda}}
\def\bXi{{\boldsymbol\Xi}}
\def\bPi{{\boldsymbol\Pi}}
\def\bSigma{{\boldsymbol\Sigma}}
\def\bUps{{\boldsymbol\Upsilon}}
\def\bPhi{{\boldsymbol\Phi}}
\def\bPsi{{\boldsymbol\Psi}}
\def\bOmega{{\boldsymbol\Omega}}

\def\ba{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\bc{\mathbf{c}}
\def\bbd{\mathbf{d}}
\def\bd{{\sf bd}}
\def\be{\mathbf{e}}
\def\bbf{\mathbf{f}}
\def\bg{\mathbf{g}}
\def\bh{\mathbf{h}}
\def\bi{\mathbf{i}}
\def\bj{\mathbf{j}}
\def\bk{\mathbf{k}}
\def\bl{\mathbf{l}}
% \def\bm{\mathbf{m}}
\def\bn{\mathbf{n}}
\def\bo{\mathbf{o}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bs{\mathbf{s}}
\def\bt{\mathbf{t}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}
\def\bw{\mathbf{w}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}

\def\balpha{{\boldsymbol\alpha}}
\def\bbeta{{\boldsymbol\beta}}
\def\bgamma{{\boldsymbol\gamma}}
\def\bdelta{{\boldsymbol\delta}}
\def\beps{{\boldsymbol\epsilon}}
\def\bveps{{\boldsymbol\varepsilon}}
\def\bzeta{{\boldsymbol\zeta}}
\def\bfeta{{\boldsymbol\eta}}
\def\btheta{{\boldsymbol\theta}}
\def\bvtheta{{\boldsymbol\vartheta}}
\def\biota{{\boldsymbol\iota}}
\def\bkappa{{\boldsymbol\kappa}}
\def\blambda{{\boldsymbol\lambda}}
\def\bmu{{\boldsymbol\mu}}
\def\bnu{{\boldsymbol\nu}}
\def\bxi{{\boldsymbol\xi}}
\def\bpi{{\boldsymbol\pi}}
\def\brho{{\boldsymbol\rho}}
\def\bvrho{{\boldsymbol\varrho}}
\def\bsigma{{\boldsymbol\sigma}}
\def\btau{{\boldsymbol\tau}}
\def\bups{{\boldsymbol\upsilon}}
\def\bphi{{\boldsymbol\phi}}
\def\bvphi{{\boldsymbol\varphi}}
\def\bpsi{{\boldsymbol\psi}}
\def\bomega{{\boldsymbol\omega}}

\def\bbA{\mathbb{A}}
\def\bbB{\mathbb{B}}
\def\bbC{\mathbb{C}}
\def\bbD{\mathbb{D}}
\def\bbE{\mathbb{E}}
\def\bbF{\mathbb{F}}
\def\bbG{\mathbb{G}}
\def\bbH{\mathbb{H}}
\def\bbI{\mathbb{I}}
\def\bbJ{\mathbb{J}}
\def\bbK{\mathbb{K}}
\def\bbL{\mathbb{L}}
\def\bbM{\mathbb{M}}
\def\bbN{\mathbb{N}}
\def\bbO{\mathbb{O}}
\def\bbP{\mathbb{P}}
\def\bbQ{\mathbb{Q}}
\def\bbR{\mathbb{R}}
\def\bbS{\mathbb{S}}
\def\bbT{\mathbb{T}}
\def\bbU{\mathbb{U}}
\def\bbV{\mathbb{V}}
\def\bbW{\mathbb{W}}
\def\bbX{\mathbb{X}}
\def\bbY{\mathbb{Y}}
\def\bbZ{\mathbb{Z}}

\def\Ber{{\sf Ber}}
\def\bin{{\sf bin}}

\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

\def\cat{{\sf cat}}
\def\Cov{{\sf Cov}}
\def\cov{{\sf cov}}
\def\card{{\bf card}}
\def\cf{{\it cf.}}
\def\cl{{\sf cl}}
\def\complex{{\bbC}}
\def\cone{{\sf cone}}
\def\conv{{\sf conv}}
\def\deq{\overset{d}{=}}
\def\det{{\sf det}}
\def\diag{{\sf diag}}
\def\diam{{\sf diam}}
\def\dist{{\sf dist}}
\def\dom{{\sf dom}}
\def\doop{{\sf do}}
\def\dto{\overset{\sf d}{\to}}
\def\Ex{{\bbE}}
\def\Exp{{\sf Exp}}
\def\exp{{\sf exp}}
\def\eg{{\it e.g.}}
\def\epi{{\sf epi}}
\def\eps{{\epsilon}}
\def\etc{{\it etc.}}
\def\ie{{\it i.e.}}
\def\iid{{\sf iid}}
\def\ind{{\sf ind}}
\def\intr{{\sf int}}
\def\integers{{\bbZ}}

\def\halpha{\widehat{\balpha}}
\def\hbeta{\widehat{\bbeta}}
\def\hdelta{\widehat{\bdelta}}
\def\hGamma{\widehat{\bGamma}}
\def\hgamma{\widehat{\bgamma}}
\def\hmu{\widehat{\bmu}}
\def\hSigma{\widehat{\bSigma}}
\def\hsigma{\widehat{\bsigma}}
\def\hTheta{\widehat{\bTheta}}
\def\htheta{\widehat{\btheta}}
\def\hw{\widehat{\bw}}

\def\KL{{\sf KL}}
\def\ker{{\sf ker}}
\def\lspan{{\sf span}}
\def\maximize{{\sf maximize}}
\def\med{{\sf med}}
\def\minimize{{\sf minimize}}
\def\norm#1{\left\|#1\right\|}
\def\ones{\mathbf{1}}
\def\Poi{{\sf Poi}}
\def\Pr{{\bbP}}
\def\peq{\overset{\sf p}{=}}
\def\plim{{\sf plim}}
\def\proj{{\sf proj}}
\def\prox{{\sf prox}}
\def\pto{\overset{\sf p}{\to}}
\def\ran{{\sf ran}}
\def\rank{{\sf rank}}
\def\reals{{\bbR}}
\def\relint{{\sf relint}}
\def\sign{{\sf sign}}
\def\supp{{\sf supp}}
\def\symm{{\bbS}}

\def\st{\textrm{subject to}}
%\def\tr{{\sf tr}}
\def\tube{{\sf tube}}
\def\TV{{\sf TV}}
\def\unif{{\sf unif}}
\def\Var{{\sf Var}}
\def\var{{\sf var}}
\def\vct{{\sf vec}}
\def\veps{\varepsilon}
\def\vol{{\sf vol}}
\def\zeros{\mathbf{0}}


==> YK-thm-macros.tex <==

\newtheorem{theorem}{Theorem}[section]
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{model}[theorem]{Model}
% \newenvironment{proof}{\noindent {\sc Proof:}}{$\Box$ \medskip} 
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}


==> exps.tex <==
\section{Computational experiments}

\subsection{Synthetic experiment setup}
\paragraph{Data distribution}
We generate the data from two group model \eqref{eq:two-groups}. Among the total $n$ number of training points $\pi$ proportion of them belongs to the majority group $g = 1$ (\ie, \ $n_1 = \lfloor n\pi\rfloor$) and the rest are from the minority group $g = 0$ ($n_0 = n - \lfloor n\pi\rfloor$).

The features $x$ in each groups are $10$ dimensional vectors generated from multivariate standard normal distribution. The response are generated from \eqref{eq:two-groups} where $\beta_0$ and $\delta$ are specified as \[ \beta_0 = \frac{r_\beta}{\sqrt 5} (\mathbf{1}_5^T, \mathbf{0}_5^T)^T, \quad \delta = \frac{r_\delta}{\sqrt 5} (\mathbf{0}_5^T, \mathbf{1}_5^T)^T \]
In all our experiments we fix total number of training points $n$ to $900$ and the majority group proportion $\pi$ to $0.9.$ In the study of \emph{sub-population shift ratio} (SSR) (defined as $ r_{\beta:\delta} = r_\beta/r_\delta$) we fix $r_\beta = 5$ and $\sigma = 0.1.$ In the study of \emph{noise} ($\sigma$)  we fix $r_\beta = 5$ and $r_\delta = 1.$ 
\paragraph{Model}
In each of the setups we fit a neural net with single hidden layer $\text{ReLU}(Wx)\in \reals^p$, where $W\in\reals^{p \times 10}$ is a random matrix \cite{mei2019generalization}. Furthermore, the final layer doesn't have the bias variable (bias is set at zero). As one might see the only unknowns of this model are the weights of the final layer, which are obtained from ridgeless regression \cite{hastie2019Surprises} with $\text{ReLU}(Wx_i)$'s as features and $y_i$'s as responses. 

\begin{figure}
    \centering
    \includegraphics[width=1.0\textwidth]{figs/ERM.pdf}
    \caption{\emph{Mean squared prediction error} (MSPE) of majority and minority groups are plotted against $\gamma = p/n$ (over 500 repetitions). The \emph{left} shows MSPE for several \emph{sub-population shift ratio} ($r_{\beta:\delta}$), whereas the same for different \emph{noise level} ($\sigma$) is shown \emph{right} panel.}
    \label{fig:mse-erm}
\end{figure}

% We generate data from the two groups model \eqref{eq:two-groups} wtih $\pi = 0.9$, $\Sigma = I_d$. In the first simulation, we set $\beta_0$ and $\beta_1 = \beta_0. \delta$ to be random unit vectors. We set $n = 200$ and vary $\gamma$ in $[1,10]$. Figure \ref{fig:bias} shows the (observed) bias and limiting bias \eqref{eq:limiting-bias} due to the difference between regression vectors. We see that the bias decreases as the aspect ratio $\gamma$ grows.

% \begin{figure}
%   \centering
% %   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
% %   \includegraphics[width=0.48\textwidth]{figs/bias-semilogy.png}
% %   ~
%   \includegraphics[width=0.48\textwidth]{figs/small-beta0-bias.png}
%   \caption{Bias and limiting bias \eqref{eq:limiting-bias} due to difference between regression vectors}
%   \label{fig:bias}
% \end{figure}

% In the second simulation, we generate set $\delta$ to be a random unit vector and study the prediction error with a small and a large values of $\beta_0$. The small $\beta_0$ setup is identical to the first simulation setup. In the large $\beta_0$ setup, we set $\beta_0$ to be a random norm 10 vector. The rest of the setup is identital to the first simulation setup. Figure \ref{fig:PE} shows the (observed) prediction error and limiting prediction error. We see that the prediction error decreases in the small $\beta_0$ setup, but it increases in the large $\beta_0$ setup.

% \begin{figure}
%   \centering
% %   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
%   \includegraphics[width=0.48\textwidth]{figs/small-beta0-PE.png}
%   ~
%   \includegraphics[width=0.48\textwidth]{figs/big-beta0-PE.png}
%   \caption{Prediction error and limiting prediction error with a small (left) and large (right) value of $\beta_0$}
%   \label{fig:PE}
% \end{figure}


% \[
% \begin{aligned}
% \begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix}^T(XX^T)^{-1}\begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix} &= X_1^T(X_1(I - X_0^\dagger X_0)X_1^T)^{-1}X_1 \\
% &= X_1^T(X_1(I - \hSigma_0^\dagger\hSigma_0)X_1^T)^{-1}X_1 \\
% &= \lim\nolimits_{z\to 0_+}X_1^T(X_1(I - (\hSigma_0 + zI_d)^{-1}\hSigma_0)X_1^T)^{-1}X_1 \\
% &= \lim\nolimits_{z\to 0_+}X_1^T(zX_1(\hSigma_0 + zI_d)^{-1}X_1^T)^{-1}X_1 \\
% &= \lim\nolimits_{z\to 0_+}\frac1zX_1^T(X_1^\dagger)^T(\hSigma_0 + zI_d)X_1^\dagger X_1.
% \end{aligned}
% \]
% Thus the second term is
% \[
% \lim\nolimits_{z\to 0_+}\frac1z\tr(\tdelta_1\tdelta_1^T(\hSigma_0 + zI_d)),
% \]
% where $\tdelta_1 \triangleq X_1^\dagger X_1\delta$. 


% \subsection{Simulation2}
% We fit single hidden layer neural-net on data generated from linear regression setup. The two groups are indexed by $g\in \{1, -1\}$, $-1$ being the minority group. We fix $\beta = \text{SNR} \times  (1, 1, 1, 1, 1, 0, 0, 0, 0, 0)^T$ and $\delta = (0, 0, 0, 0, 0, 1, 1, 1, 1, 1)$. The pair $(x^{(g)}, y^{(g)})$ is generated from the following distribution. \begin{equation}
%     \left\{ \begin{aligned}
%     x^{(g)} & \sim N_{10}(0, I_{10})\\
%     y^{(g)} & \sim N\left(\left({x^{(g)}}\right)^T \beta_g, \sigma^2\right)
%     \end{aligned} \right.
% \end{equation} 
% The training data consists of 2000 independent pairs, where 90\% of them are from group 1 and 10\% are from group -1. We fit single hidden layer neural network with various number of nodes. NNs are trained with weighted sample points to account for class imbalance in training data. 
% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\textwidth]{figs/plot.pdf}
%     \caption{Prediction error   }
%     \label{fig:mse-nn}
% \end{figure}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> theory.tex <==
\section{Theoretical study of inversion map}

\subsection{Assumptions}

\paragraph{Generative process}

Let us assume that latent space $\cZ = \cZ_S \times \cZ_{S^{c}} \subset \reals^d$ where $S \subset [d]$, $\cZ_S = \{z_S \in \reals^{|S|}: \|z_S\|_2 = 1 \}$, $\cZ_{S^c} = \{z_{S^c} \in \reals^{|S^c|}: \|z_{S^c}\|_2 = 1\}$. The latent space can be rewritten as $\cZ = \{z \equiv (z_S, z_{S^c}) \in \reals^d: \|z_S\|_2 = 1, \|z_{S^c}\|_2 = 1\}$. Let $g : \cZ \to \cX \subset \reals^K$ be the generator map, where $K \ge d$ where $g$ is an injective map and differentiable in the vicinity (an open cover) of $\cZ$. Here, we assume that the $S$ co-ordinates are associated with some properties $P$, \ie, any change in the co-ordinates will reflect changes in the properties $P$ for the $x$-samples. We assume that the marginal distribution $p(z)$ over the latent space is uniform: 
\begin{equation}
    p(z) = \frac{1}{|\cZ|} \bI\{z \in \cZ\}\,.
\end{equation}
We further assume that the conditional distribution over the positive/similar pairs for $S$ and $S^c$ (a modified version of the von Mises-Fisher(vMF) distribution): 
\begin{equation}
% \label{eq:loss}
    p_S(z^{+} | z) = C_S^{-1}  e^{\kappa \langle z_S, z_S^{+} \rangle }, ~~ p_{S^c}(z^{+} | z) = C_{S^c}^{-1}  e^{\kappa \langle \zsc, \zscp \rangle }
\end{equation} where $C_S = \int_{\cZ}e^{\kappa \langle z_S, z_S^{+} \rangle } \zp $ and $C_{S'} = \int_{\cZ}e^{\kappa \langle \zsc, \zscp \rangle } \zp$. The negative samples are always generated independently as $z'\sim p(z)$. \todo[inline]{fix constants: correct integration spaces and only integrate the density}

\paragraph{Model} Let $f : \cX \to \cZ' \triangleq\Zs'\times \Zsc'$ where $\Zs' = \{z_S\in \reals^{|S|}: \|z_S\|_2 = 1\}$ and $\cZ_{S^c}' = \{z_{S^c} \in \reals^{|S^c|}: \|z_{S^c}\|_2 = 1\}$. The parameter $f$ of the problem is optimized via a contrastive learning algorithm (TBD). We associate two conditional distributions $q_{h, S}(\zp\mid z)$ and $q_{h, S^c}(\zp \mid z)$ with our model $f$ through $h = f \circ g$ and \begin{equation}
\begin{aligned}
    q_{h, T}(\zp\mid z) =   C_{h, T}(z)^{-1} e^{\gamma \langle h(z)_T, h(z^{+})_T \rangle}\\
    \text{with} ~~  C_{h, T}(z) = \int e^{\gamma \langle h(z)_T, h(z^{+})_T \rangle} d\zp, ~~\text{and} ~~ T = S, S^c
\end{aligned}
\end{equation}

We now define the constrastive objective. Let $z, z'_{1, 1}, \dots, z'_{1, M_1}, z'_{2, 1}, \dots, z'_{2, M_{2}}$ be independently drawn samples from $p$. We furthermore generate two positive samples, $\zp_1 \sim p_S(z^{+} | z)$ and $\zp_2 \sim p_{S^c}(z^{+} | z)$ \todo[inline]{This is ambiguous, since the samples are actually in the product space and the distributions are over the component spaces}. Note that, $\zp_1$ and $\zp_2$ are similar to $z$ in terms of $S$ and $S^c$ co-ordinates. As an example, for an image $z$ which is uniformly drawn and is uniformly blurred, $\zp_1$ could be an different (uniformly drawn) image with same blurring and $\zp_2$ is the same image with different (uniformly drawn) blurring.  Letting $x, x'_{1, 1}, \dots, x'_{1, M_1}, x'_{2, 1}, \dots, x'_{2, M_2}$, $x_1^{+}, x_2^+$ are corresponding $x$-samples we define the two-part contrastive loss as:
\begin{equation}
\begin{aligned}
&\min_f L_{\text{contr}}(f)~~ \text{subject to} ~~ \|f_S(x)\|_2 = 1, \|f_{S^c}\|_2 = 1, \\
 & \text{where} ~~  L_{\text{contr}}(f) = L_{\text{contr}, S}(f) + L_{\text{contr}, S^c}(f), \\
  &  L_{\text{contr}, S}(f, \gamma_1, M_1) =  \Ex_{\substack{z, z'_{1, 1}, \dots, z'_{1, M_1} \sim p(z),\\ \zp_1 \sim p_S(z^{+} | z)}} \left[- \log \bigg\{\frac{e^{\gamma_1 \langle h(z)_S, h(z_1^{+})_S \rangle}}{e^{\gamma_1 \langle h(z)_S, h(z_1^{+})_S \rangle} + \sum_{i = 1}^{M_1} e^{\gamma_1 \langle h(z)_S, h(z_{1, i})_S \rangle}}\bigg\}\right]\\
 &   L_{\text{contr}, {S^c}}(f, \gamma_2, M_2) =  \Ex_{\substack{z, z'_{2, 1}, \dots, z'_{2, M_2} \sim p(z),\\ \zp_2 \sim p_{S^c}(z^{+} | z)}} \left[- \log \bigg\{\frac{e^{\gamma_2 \langle h(z)_{S^c}, h(z_2^{+})_{S^c} \rangle}}{e^{\gamma_2 \langle h(z)_{S^c}, h(z_2^{+})_{S^c} \rangle} + \sum_{i = 1}^{M_2} e^{\gamma_2 \langle h(z)_{S^c}, h(z_{2, i})_{S^c} \rangle}}\bigg\}\right]
\end{aligned}
\label{eqn:contrastive_objective}
\end{equation}

\todo[inline]{Would be useful in main body to restate the objectives and optimization problem in terms of the training data $x$ and the inversion model $f$, as that is how readers will implement~\ref{eqn:contrastive_objective}. Then this formulation may be more convenient for the appendix when you're actually proving things.}

\todo[inline]{In~\ref{eqn:contrastive_objective}, would be helpful to note/clarify that sampling $z_1^+$, a $d$-dimensional code, from $p_S(z^+ | z)$, a distribution on a less than $d$-dimensional space, refers to sampling the $S$ coordinates from that distribution and the remaining $S^c$ coordinates from the uniform distribution on $\mathcal{Z}_{S^c}$. Likewise for the negative sampling in the second contrastive loss.}


\begin{algorithm}[!t]
\caption{\label{alg:main} DiCLR's learning algorithm.}
\begin{algorithmic}
    \STATE \textbf{input:} batch size $N$, constant $\tau$, structure of $f$, transformation ensemble $\mathcal{T}$.
    \FOR{sampled minibatch $\{\bm x_k\}_{k=1}^N$}
    \STATE draw augmentation function $t \!\sim\! \mathcal{T}$
    \STATE \textbf{for all} $k\in \{1, \ldots, N\}$ \textbf{do}
        \STATE $~~~~$draw augmentation function $t \!\sim\! \mathcal{T}$ 
        \STATE $~~~~$${\bm h}_k = f({\bm x}_k)$ \textcolor{gray}{~~~~~~~~\# latent code for k-th image}
        \STATE $~~~~$$\tilde {\bm h}_k = f(t({\bm x}_k))$ \textcolor{gray}{~~~~~~~~\# latent code for transformed k-th image}
        \STATE
      %\STATE # idea: first loss function says rotated image should have similarity to a random rotated image in $S$ coordinates; second uses the regular simCLR in the $S^c$ coordinates.

 %       \STATE $~~~~$\textcolor{gray}{\# For computing $L_{\text{contr},S}$: sampling from $p_S(z^+ | z)$}
        \STATE $~~~~$draw $i_k \in \{1,\ldots, N\}\backslash\{k\}$, an index of a sample, uniformly at random

        \STATE $~~~~$$\tilde {\bm h} = f(t({\bm x}_{i_k}))$ \textcolor{gray}{~~~~~~~~\# features of the transformed positive sample}      
        \STATE $~~~~$$w_k^S = \exp\left(\gamma_1 \left\langle \tilde{\bm h_k}, \tilde {\bm h}\right \rangle_S/\|\tilde{\bm h_k}\|_S \|\tilde{\bm h}\|_S \right)$
        \STATE $~~~~$$w_k^{S^c} = \exp\left(\gamma_2 \left\langle {\bm h}_k, \tilde{\bm h}_k \right\rangle_{S^c}/\|{\bm h}_k\|_{S^c} \|\tilde{\bm h}_k\|_{S^c} \right)$
%         \STATE 
%         \STATE $~~~~$\textcolor{gray}{\# For computing $L_{\text{contr},S^c}$: sampling from $p_{S^c}(z^+ | z)$}
%
%        \STATE $~~~~$$\tilde{\bm x} = t(\bm x_k)$ 
%        \STATE $~~~~$$\bm h= f(\tilde{\bm x})$ \textcolor{gray}{~~~~~~~~\# features of the second transformed positive sample}      
%        \STATE $~~~~$$w_k^{S^c} = \exp\left(\gamma_2 \left\langle \bm h_k, {\bm h}\right \rangle_{S^c}/\|\bm h_k\|_{S^c} \|\bm h\|_{S^c} \right)$
    \STATE \textbf{end for}
    \STATE \textbf{for all} $(j,k)\in\{1, \ldots, N\}^2$ \textbf{do}
    \STATE $~~~~$ $c_S(j, k) = \exp\left(\gamma_1 \langle \bm h_j, \bm h_k \rangle_{S}/ \|\bm h_j\|_S \|\bm h_k\|_S \right)$
    \STATE $~~~~$ $c_{S^c}(j,k) = \exp\left(\gamma_2 \langle \bm h_j, \bm h_k \rangle_{S^c}/ \|\bm h_j\|_{S^c} \|\bm h_k\|_{S^c} \right)$
    \STATE \textbf{end for}
    \STATE \textbf{define} $\ell_S(k)$ as $\ell_S(k) = -\log\left(\frac{w_k^S }{w_k^S + \sum_{\ell = 1}^N \mathbbm{1}_{\ell \neq k} c_S(k, \ell) } \right)$
    \STATE \textbf{define} $\ell_{S^c}(k)$ as $\ell_{S^c}(k) = -\log\left(\frac{w_k^{S^c} }{w_k^{S^c} + \sum_{\ell = 1}^N \mathbbm{1}_{\ell \neq k} c_{S^c}(k, \ell) } \right)$
    \STATE $\mathcal{L} = \frac{1}{N} \sum_{k=1}^N \left[ \ell_S(k) + \ell_{S^c}(k)\right]$
    \STATE update network $f$ to minimize $\mathcal{L}$
    \ENDFOR
    \STATE \textbf{return} encoder network $f(\cdot)$
\end{algorithmic}
\end{algorithm}


\begin{proposition}[\cite{zimmermann2021contrastive}, Proposition A]
\label{prop:loss-split}
As the numbers of samples $M_1, M_2$ approach infinity, the normalized contrastive loss converges to
\begin{equation}
    \begin{aligned}
    \lim_{M_1\to \infty} L_{\textrm{contr}, S}(f, \gamma_1, M_1) - \log M_1
=  L_{\text{align}, S}(f, \gamma_1) + L_{\text{uni}, S}(f, \gamma_1) \\
\lim_{M_2\to \infty} L_{\textrm{contr}, {S^c}}(f, \gamma_2, M_2) - \log M_2
=  L_{\text{align}, {S^c}}(f, \gamma_2) + L_{\text{uni}, {S^c}}(f, \gamma_2)
\end{aligned}
\end{equation} where, for $T = S, S^c,$
\begin{equation}
    \begin{aligned}
    L_{\text{align}, T}(f, \gamma_T) = - \gamma_T \Ex_{(z, \zp) \sim p(z)p_S(\zp| z)} \big[ \langle h(z)_{T}, h(z^{+})_{T} \rangle \big]\\
    L_{\text{uni}, T}(f, \gamma_T) =\Ex_{z \sim p(z)} \bigg[\log \Ex_{z' \sim p(x)} \Big[e^{\gamma_T\langle h(z)_{T}, h(z')_{T} \rangle}\Big]\bigg]\,.
    \end{aligned}
\end{equation}

\end{proposition}

\begin{proposition}[\cite{zimmermann2021contrastive}, Theorem 1]
\label{prop:cross-ent}
For $T = S, S^c$ it holds 
\begin{equation}
    \lim_{M_1\to \infty} L_{\text{contr}, S}(f, \gamma_T, M_T) - \log M_T + \log |\cZ| = \Ex_{z \sim p(z)} [H\big(p_T(\cdot| z), q_{h, T}(\cdot| z)\big)]\,.
\end{equation}


\end{proposition}

\begin{proof}
\[
\begin{aligned}
&\Ex_{z \sim p(z)} [H\big(p_T(\cdot| z), q_{h, T}(\cdot| z)\big)]\\
= & \Ex_{z \sim p(z)} \left[\Ex_{\zp\sim p_T(\cdot| z)}\big[-\log  q_{h, T}(\cdot| z)\big]\right]\\
= & -\Ex_{(z, \zp) \sim p(z)p_T(\cdot| z)}[\gamma_T\langle h(z)_{T}, h(z^{+})_{T} \rangle] + \Ex_{z \sim p(z)} [\log C_{h, T}(z) ]\,.
\end{aligned}
\] Here, the first summand in the last expression is equal to $L_{\text{align}, T}(f, \gamma_T)$. Next we show that the other summand equates with $L_{\text{uni}, T}(f, \gamma_T) + \log |\cZ|$. From the definition of $C_{h, T}(z)$ we obtain 
\[
\begin{aligned}
&\Ex_{z \sim p(z)} [\log C_{h, T}(z) ]\\
=& \Ex_{z \sim p(z)} \left[\log \int e^{\gamma_T \langle h(z)_T, h(z^{+})_T \rangle} d\zp \right]\\
=& \Ex_{z \sim p(z)} \left[\log \int e^{\gamma_T \langle h(z)_T, h(z^{+})_T \rangle} \frac{d\zp}{|\cZ|} \right] + \log |\cZ|\\
=& \Ex_{z \sim p(z)} \left[\log \Ex_{\zp \sim p(z)}\Big[ e^{\gamma_T \langle h(z)_T, h(z^{+})_T \rangle} \Big] \right] + \log |\cZ|\\
=& L_{\text{uni}, T}(f, \gamma_T) + \log |\cZ|\,,
\end{aligned}
\] where the second last equality is obtained by noticing that $p(z) = 1/|\cZ|$. Till now we have obtained
\begin{equation}
    \Ex_{z \sim p(z)} [H\big(p_T(\cdot| z), q_{h, T}(\cdot| z)\big)] = L_{\text{align}, T}(f, \gamma_T) + L_{\text{uni}, T}(f, \gamma_T) + \log |\cZ|\,.
\end{equation} From Proposition \ref{prop:loss-split} we conclude the proof. 
\end{proof}

A conclusion of Proposition \ref{prop:cross-ent} is that the minimization in the contrastive loss leads to $p_T(\cdot| z) = q_{h, T}(\cdot| z)$ for $T \in \{S, S^c\}$. 

\begin{proposition}
\label{prop:isometry}
$p_T(\cdot| z) = q_{h, T}(\cdot| z)$ for $T \in \{S, S^c\}$ implies for all $z, z'\in \cZ$ it holds $ \langle h(z)_T, h(z')_T \rangle = \langle z_T, z'_T \rangle$.
\end{proposition}

\begin{proof}
A conclusion of $p_T(\cdot| z) = q_{h, T}(\cdot| z)$ is $p_T(z| z) = q_{h, T}(z| z)$ which follows
\[
\begin{aligned}
&C_T^{-1} e^{\kappa\langle z_T, z_T \rangle}  =  C_{h, T}(z)^{-1} e^{\gamma_1\langle h(z)_T, h(z)_T \rangle} \\
\iff & C_T  =  C_{h, T}(z)
\end{aligned}
\] where noticing that  $\langle z_T, z_T \rangle = \langle h(z)_T, h(z)_T \rangle = 1$  the last inequality hold for $\gamma_T = \kappa$.
\end{proof}

\begin{proposition}
Let $h: \cZ \to \cZ$ be a differentiable map that satisfies $ \langle h(z)_T, h(z')_T \rangle = \langle z_T, z'_T \rangle$ for $T \in \{S, S^c\}$. Then $h(z) = R z$ where $R$ is a block diagonal orthogonal matrix of the form:  $R_{S, S} \in \reals^{|S| \times |S|}$ and $R_{S^c, S^c} \in \reals^{|S^c| \times |S^c|}$ are orthogonal matrices and $R_{S, S^c} = 0$, $R_{S^c, S} = 0$. 
\end{proposition}
\begin{proof}
Fix $T \in \{S, S^c\}$ and define $J_T(z) = \frac{\partial h_T}{z_T}(z) \in \reals^{|T| \times |T|}$. We differentiate both sides of $\langle h(z)_T, h(z')_T \rangle = \langle z_T, z'_T \rangle$ with respect to $z$ to obtain 
\begin{equation}
    J_T(z)^\top h(z')_T = z'_T\,.
\end{equation} We now differentiate both sides with respect to $z'$ and obtain that for any $z, z' \in \cZ$
\begin{equation}
    J_T(z)^\top J_T(z') = I ~~ \text{or} ~~ J_T(z)^\top = J_T(z')^{-1}\,.
\end{equation} The above identity implies that  $J_T(z)$ is a constant matrix and it's orthogonal. Hence, $h^T(z) = R_{T, T} z_T$ for some orthogonal matrix $R_{T, T} \in \reals^{|T| \times |T|}$, which concludes the lemma. 

\end{proof}


\subsection{Theory for post-processing}

Let us assume that the latent space $\cZ \in \reals^d$ and the latent samples are drawn from the latent distribution $z \sim p(z)$. We further assume that there exist a generative map $g: \reals^d \to \reals^N$ such that for a generic $z \in \cZ$ a sample is created as $x = g(z) \in \reals^N$. We assume that we have access to a map $f: \reals^N \to \cZ$ such that  $f \circ g(z) = Az$ for all $z \in \cZ$ and some invertible matrix $A\in \reals^{d \times d}$ which is independent of $z$. We fix an $S \subset [d]\triangleq \{1, \dots, d\}$ and assume that for any $x = g(z)$ we have access to the modified images $\{x_j' = g(z_j'): j \in S\}$ where 
\begin{equation}
    z_j' = \begin{cases}
    [z_j']_i = [z]_i & i \neq j,\\
    [z_j']_i = - [z]_i & i = j.
    \end{cases}
\end{equation} For the simplicity of notations (without loss of generality) we assume $S = [m]$ where $m = |S|$. Given samples $\{x_i\}_{i = 1}^n$ we first obtain the direction corresponding to the $j$-th ($j \le m$) latent co-ordinate as a solution to the following linear regression problem: 
\begin{equation}
% \label{eq:jth-direction}
\begin{aligned}
\hat \beta_j  = \beta_j / \|\beta_j\|_2,\\
(\alpha_j, \beta_j) = \argmin_{(\alpha, \beta)} \frac{1}{2n} \Big[\sum_{i = 1}^n \big\{\alpha + \beta^\top f(x_i) - 1\big\}^2 + \sum_{i = 1}^n \big\{\alpha + \beta^\top f\big({(x_i)}_j'\big) + 1\big\}^2\Big]
\end{aligned}
\end{equation}

\begin{lemma}
\emph{The lemma goes in supplement.} Let $p(z)$ is a rotationally invariant distribution, \ie, \ if $Z \in p(z)$ then for any orthogonal matrix $R \in \reals^{d \times d}$ it holds:  $Z \stackrel{d}{=} RZ$. Then for $Z \sim p(z)$ we have 1. $\Ex[Z] = 0$, and 2. $\text{var}(Z) = r^2 I_d$, for some $r> 0$. 
\end{lemma}

\begin{proof}
\emph{1.} Since $Z \sim  p(z)$  rotationally invariant we have $Z \stackrel{d}{=} - Z$ which implies $\Ex [Z] = \Ex[-Z]$ or $\Ex [Z] = 0$. 

\emph{2.}  From \emph{1.} we see that $\text{var}[Z] = \Ex [ZZ^\top ] = \big[\Ex[Z_iZ_j]\big]_{i, j \in [d]}$.  Since $Z \stackrel{d}{=} ([Z_1], \dots, [Z_{i - 1}], - [Z_i], [Z_{i + 1}], \dots, [Z_d])^\top$ due to rotational invariance,  then $\Ex[Z_iZ_j] = \Ex[-Z_iZ_j]$ as long $i \neq j$ and this follows $\Ex[Z_iZ_j] = 0$. On the other hand, noticing that $([Z_1], \dots, [Z_{i - 1}],  [Z_i], [Z_{i + 1}], \dots, [Z_d])^\top \stackrel{d}{=} ([Z_1], \dots, [Z_{i - 1}],  [Z_1], [Z_{i + 1}], \dots, [Z_d])^\top$ we conclude $\Ex[Z_i^2] = \Ex[Z_1^2] = r^2$ for some $r>0$. This concludes the lemma. 





\end{proof}

To this point we assume that the latent distribution is rotationally invariant, \ie, if $Z \sim p(z)$ then for any orthogonal matrix $O\in \reals^{d \times d}$ the random variables $Z $ and $ OZ$ are equally distributed.

We also mention that any matrix $A$ can be written as $A = TO$ for an upper triangular matrix $T$ and an orthogonal matrix $O$. Since $A$ is an invertible matrix, so is $T$. We define $r_j \triangleq \{T^\top\}^{-1} o_j$ and note that $r_j^\top A = e_j^\top$ where $\{e_i\}_{i = 1}^{d}$ is the canonical basis for $\reals^d$. 
In the next lemma we show that the limiting values of latent co-ordinate directions $\hat \beta_j$ coincides with $r_j$. 

\begin{lemma}
Let $\{x_i = g(z_i)\}_{i = 1}^n$ where $z_i \sim p(z)$ and  $\hat \beta_j = \hat \beta_j^{(n)}$ is calculated as in \eqref{eq:jth-direction}. If $p(z)$ is rotationally invariant then $  \frac{|r_j^\top {\hat\beta_j^{(n)}} |}{\|r_j\|_2}\stackrel{a.s.}{\longrightarrow} 1 $.
\end{lemma}

\begin{proof}
Define $u_i \triangleq f(x_i) = A z_i$ and $u_{n+i} \triangleq f\big( (x_i)_j' \big) = A (z_i)_j'$ and 
\begin{equation}
    v_i = \begin{cases}
    1 & i = 1, \dots, n,\\
    -1 & i = n+ 1, \dots, 2n. 
    \end{cases}
\end{equation} We further define $\bar u = \frac 1{2n}\sum_{i = 1}^{2n} u_i$ and $\bar v = \frac 1{2n}\sum_{i = 1}^{2n} v_i = 0$. Then 
\[
\beta_j^{(n)} = \Big\{ \frac 1{2n}\sum_{j = 1}^{2n} (u_i - \bar u)(u_i - \bar u)^\top \Big\}^{-1} \Big\{ \frac 1{2n}\sum_{j = 1}^{2n} (u_i - \bar u)v_i \Big\}\,.
\] Here, 
\[
\bar u = \frac12 \Big(\frac1n \sum_{i = 1}^n u_i + \frac1n \sum_{i = 1}^n u_{n+i}\Big) =  A\frac12 \Big(\frac1n \sum_{i = 1}^n z_i + \frac1n \sum_{i = 1}^n (z_i)_{j}'\Big) \stackrel{a.s.}{\longrightarrow} 0\,.
\] and 
\[
\begin{aligned}
\frac 1{2n}\sum_{j = 1}^{2n} (u_i - \bar u)(u_i - \bar u)^\top & =
\frac{1}{2n} \sum_{i = 1}^n u_i u_i^\top + \frac1{2n} \sum_{i = 1}^n u_{n+i} u_{n+i}^\top -  \bar u \bar u^\top \\
& = A \Big\{\frac{1}{2n} \sum_{i = 1}^n z_i z_i^\top\Big\} A^\top  + A \Big\{\frac1{2n} \sum_{i = 1}^n (z_i)_j' \{(z_i)_j'\}^\top \Big\} A^\top -  \bar u \bar u^\top\\
& \stackrel{a.s.}{\longrightarrow} r^2 AA^\top = r^2 TT^\top  \,.
\end{aligned}
\] We further notice that 
\[
\begin{aligned}
\frac 1{2n}\sum_{j = 1}^{2n} (u_i - \bar u) v_i &= \frac{1}{2n} \sum_{i = 1}^n (u_i - u_{n+i})  - \frac{1}{2n} \bar u\Big( \cancelto{0}{\sum_{i = 1}^n v_i}\Big)\\
& = \frac{1}{2n} \sum_{i = 1}^n A (z_i - (z_i)_j')\\
& = \frac{1}{2n} \sum_{i = 1}^n T O (z_i - (z_i)_j')\\
& = \frac{1}{2n} \sum_{i = 1}^n   2 T o_j [z_i]_j\\
& = T o_j [\bar z]_j
\end{aligned}
\] which implies 
\[
\begin{aligned}
\beta_j^{(n)} &= \Big\{ \frac 1{2n}\sum_{j = 1}^{2n} (u_i - \bar u)(u_i - \bar u)^\top \Big\}^{-1} T o_j [\bar z]_j\,.
\end{aligned}
\]
We now look at $\hat \beta_j^{(n)}$ which can be written as: 
\[
\begin{aligned}
\hat \beta_j^{(n)} & = \frac{\beta_j^{(n)}}{\|\beta_j^{(n)}\|_2}\\
& = \frac{\Big\{ \frac 1{2n}\sum_{j = 1}^{2n} (u_i - \bar u)(u_i - \bar u)^\top \Big\}^{-1} T o_j [\bar z]_j}{\sqrt{o_j^\top T^\top  [\bar z]_j\Big\{ \frac 1{2n}\sum_{j = 1}^{2n} (u_i - \bar u)(u_i - \bar u)^\top \Big\}^{-2} T o_j [\bar z]_j}}\\
& = \frac{\Big\{ \frac 1{2n}\sum_{j = 1}^{2n} (u_i - \bar u)(u_i - \bar u)^\top \Big\}^{-1} To_j \text{sign}([\bar z]_j)}{\sqrt{o_j^\top T^\top \Big\{ \frac 1{2n}\sum_{j = 1}^{2n} (u_i - \bar u)(u_i - \bar u)^\top \Big\}^{-2} To_j }}
\end{aligned}
\] which means 
\[
\begin{aligned}
|o_j^\top T^{-1} \hat \beta_j^{(n)}| & = \frac{\left|o_j^\top T^{-1} \Big\{ \frac 1{2n}\sum_{j = 1}^{2n} (u_i - \bar u)(u_i - \bar u)^\top \Big\}^{-1} To_j \text{sign}([\bar z]_j)\right|}{\sqrt{o_j^\top T^\top \Big\{ \frac 1{2n}\sum_{j = 1}^{2n} (u_i - \bar u)(u_i - \bar u)^\top \Big\}^{-2} To_j }}\\
& = \frac{\left|o_j^\top T^{-1} \Big\{ \frac 1{2n}\sum_{j = 1}^{2n} (u_i - \bar u)(u_i - \bar u)^\top \Big\}^{-1} To_j \right|}{\sqrt{o_j^\top T^\top \Big\{ \frac 1{2n}\sum_{j = 1}^{2n} (u_i - \bar u)(u_i - \bar u)^\top \Big\}^{-2} To_j }}\\
& \stackrel{a.s.}{\longrightarrow} \frac{\left|o_j^\top T^{-1} \Big\{ r^2 TT^\top  \Big\}^{-1} To_j \right|}{\sqrt{o_j^\top T^\top \Big\{ r^2 TT^\top \Big\}^{-2} To_j }}\\
& = \frac{\left|o_j^\top T^{-1} \Big\{ \cancel{r^2} TT^\top  \Big\}^{-1} To_j \right|}{\sqrt{o_j^\top T^\top \Big\{ \cancel{r^2} TT^\top \Big\}^{-2} To_j }}\\
& = \frac{\left|o_j^\top T^{-1} \{T^{-1}\}^\top T^{-1}  To_j \right|}{\sqrt{o_j^\top T^\top \{T^{-1}\}^\top T^{-1}\{T^{-1}\}^\top T^{-1} To_j }}\\
& = \frac{\left|o_j^\top T^{-1} \{T^{-1}\}^\top o_j \right|}{\sqrt{o_j^\top  T^{-1}\{T^{-1}\}^\top o_j }} = \|\{T^{-1}\}^\top o_j\|_2 = \|r_j\|_2 \,.
\end{aligned}
\]

\end{proof}
